DRCT: Saving Image Super-resolution away from Information Bottleneck

In recent years, Vision Transformer-based approaches for low-level vision tasks have achieved widespread success. Unlike CNN-based models, Transformers are more adept at capturing long-range dependencies, enabling the reconstruction of images utilizing non-local information. In the domain of super-resolution, Swin-transformer-based models have become mainstream due to their capability of global spatial information modeling and their shifting-window attention mechanism that facilitates the interchange of information between different windows. Many researchers have enhanced model performance by expanding the receptive fields or designing meticulous networks, yielding commendable results. However, we observed that it is a general phenomenon for the feature map intensity to be abruptly suppressed to small values towards the network's end. This implies an information bottleneck and a diminishment of spatial information, implicitly limiting the model's potential. To address this, we propose the Dense-residual-connected Transformer (DRCT), aimed at mitigating the loss of spatial information and stabilizing the information flow through dense-residual connections between layers, thereby unleashing the model's potential and saving the model away from information bottleneck. Experiment results indicate that our approach surpasses state-of-the-art methods on benchmark datasets and performs commendably at the NTIRE-2024 Image Super-Resolution (x4) Challenge. Our source code is available at https://github.com/ming053l/DRCT

==> sec/0_abstract.tex <==
\begin{abstract}

In recent years, Vision Transformer-based approaches for low-level vision tasks have achieved widespread success. Unlike CNN-based models, Transformers are more adept at capturing long-range dependencies, enabling the reconstruction of images utilizing non-local information. In the domain of super-resolution, Swin-transformer-based models have become mainstream due to their capability of global spatial information modeling and their shifting-window attention mechanism that facilitates the interchange of information between different windows. Many researchers have enhanced model performance by expanding the receptive fields or designing meticulous networks, yielding commendable results. However, we observed that it is a general phenomenon for the feature map intensity to be abruptly suppressed to small values towards the network's end. This implies an information bottleneck and a diminishment of spatial information, implicitly limiting the model's potential. To address this, we propose the Dense-residual-connected Transformer \textbf{(DRCT)}, aimed at mitigating the loss of spatial information through dense-residual connections between layers, thereby unleashing the model's potential and saving model away from information bottleneck. Experiment results indicate that our approach surpasses state-of-the-art methods on benchmarks dataset and performs commendably at NTIRE-2024 Image Super-Resolution (x4) Challenge. 
\end{abstract}

==> sec/2_5_problemformulation.tex <==
\section{Problem Statement}
\label{sec:Problem}
\begin{figure*}
    \begin{center}
    \includegraphics[width=1\textwidth]{fig/DRCT9.png}
    \end{center}
    \caption{The overall architecture of the proposed DRCT and the structure of RDG and SDRCB.}
     \label{DRCT.png}
\end{figure*}

\subsection{Information Bottleneck Principle}

According to the information bottleneck principle \cite{IBP}, the given data \(X\) may cause information loss when going through consecutive layers. It may lead to gradient vanish when back-propagation for fitting network parameters and predicting \(Y\), as shown in the equation below:
\begin{equation}
I(X, X) \geq I(Y, X) \geq I(Y, f_{\theta}(X)) \geq I(X, g_{\phi}(f_{\theta}(X))),
\label{equation1}
\end{equation}
where \(I\) indicates mutual information, \(f\) and \(g\) are transformation functions, and \(\theta\) and \(\phi\) are parameters of \(f\) and \(g\), respectively.

In deep neural networks, \(f_{\theta}(\cdot)\) and \(g_{\phi}(\cdot)\) respectively represent the two consecutive layers in neural network. From equation (\ref{equation1}), we can predict that as the number of network layer becomes deeper, the original data will be more likely to be lost. In term of SISR tasks, the general goal is to find the mapping function $F$ with optimized function parameters $\theta$ to maximize the mutual information between HR and SR image.

\begin{equation}
    F(\mathbf{I}_{LR}; \theta) = \mathbf{I}_{SR}; \\
    \max_{\theta} I(\mathbf{I}_{HR}; F(\mathbf{I}_{LR}; \theta))
\end{equation}


\subsection{Spatial Information Vanish in Super-resolution}

Generally speaking, SISR methods \cite{HAT,CAT,SwinIR,SwinFIR,ART,DAT,SRFormer,CRAFT} can generally divided into three parts: (1) shallow feature extraction, (2) deep feature extraction, (3) image reconstruction. 

In these methods, there is almost no difference between shallow feature extraction and image reconstruction. The former is composed of simple convolutional layers, while the latter consists of convolutional layers and upsampling layers. However, deep feature extraction differs significantly. Yet, their commonality lies in being composed of various residual blocks, which can be simply defined as:

\begin{equation}
X^{l+1} = X^{l} + f_{\theta}^{l+1}(X^{l}),
\end{equation}
where \(X\) indicates inputs, \(f\) is a consecutive layers for \(l\)'th residual group , and \(\theta\) represents the parameters of $f^{l}$.

Using residual learning allows the model to only update the differences between layers, rather than predicting the total output of a layer directly. This reduces the difficulty of model training and prevents gradient vanishing. However, according to our observations, while this design effectively transmits spatial information between different residual blocks, there may still be information loss.

Because the information within a residual block may not necessarily maintain spatial information, this ultimately leads to non-smoothness in terms of feature map intensity (refer to Fig. \ref{vanish.png} and \ref{featuremapintensity3.png}), causing an information bottleneck at the deepest layers during forward propagation. This makes it easy for spatial information to be lost as the gradient flow reaches the deeper layers of the network, resulting in reduced data efficiency or the need for more complex network designs to achieve better performance.


To better evaluate information loss, the G-index is defined by the sum of two components: the absolute change in the maximum intensities and the absolute change in the minimum intensities of the feature maps. It quantifies the absolute difference in both the highest and lowest feature map intensities between two consecutive layers.

\begin{equation}
 GI = \sum^{L}_{l=1} (\left\|\Delta G_{min}^{l}\right\| + \left\|\Delta G_{max}^{l}\right\|),
\end{equation}
where \(L\) is the depth of network. G-index, encapsulating the total of these absolute changes. (refer to Figure \ref{featuremapintensity3.png}.) The proposed DRCT exhibits the smoothest changes in feature map intensity, reflecting a lower G-index. This implies that spatial information can be well preserved during the forward-propagation.

\subsection{Dense-Residual Group Auxiliary Supervision}

Motivated by RRDB-Net \cite{RRDB}, Wang \emph{et al.} suggested that incorporating dense-residual connections can aggregates multi-level feature information and stabilize training through residual learning \cite{EDSR,szegedy2016inceptionv4}. Nonetheless, CNN-based approaches, which primarily focus on learning local information, often overlook the importance of capturing long-range dependencies. Recent studies on SwinIR-based methods have concentrated on enlarging the receptive field \cite{HAT,CAT,ART,DAT} or enhancing the network's capability to extract features \cite{CRAFT,Uformer} for high-quality SR images.

By adding dense-connections \cite{huang2018densely} within Swin-Transformer-based blocks \cite{SwinIR,SwinTransformer} in SISR network for deep feature extraction, we consider that it is possible to stabilize the gradient flow within each residual-groups during back-propagation, thereby addressing the issue of information bottlenecks and enhancing the receptive field. Consequently, this approach allows for achieving outstanding performance with simpler model architectures, or even by using shallower SISR networks.

==> sec/2_related.tex <==
\section{Related works}
\label{sec:relatedworks}

\begin{figure*}
\includegraphics[width=1\textwidth]{fig/vanish2.png}
\caption{The feature map visualization displays, from top to bottom, SwinIR \cite{SwinIR}, HAT \cite{HAT}, and DRCT, with positions further to the right representing deeper layers within the network. For both SwinIR and HAT, the intensity of the feature maps is significant in the shallower layers but diminishes towards the network's end. We consider this phenomenon implies the loss of spatial information, leading to the limitation and information bottleneck with SISR tasks. (zoom in to better observe the color-bar besides feature maps.)} \label{vanish.png}
\end{figure*}


\begin{figure}
\includegraphics[width=0.48\textwidth]{fig/drct8.png}
\caption{The G-index we propose is calculated by the summation of absolute values of $\Delta G_{min}$ and $\Delta G_{max}$, where $\Delta G$ represents the change in feature map intensity between two consecutive layers. This change is measured by the difference in intensity levels, capturing both the minimum and maximum shifts across layers.} \label{featuremapintensity3.png}
\end{figure}

\subsection{Vision Transformer-based Super-Resolution}


IPT \cite{IPT}, a versatile model utilizing the Transformer encoder-decoder architecture, has shown efficacy in several low-level vision tasks. SwinIR \cite{SwinIR}, building on the Swin Transformer \cite{SwinTransformer} encoder, employs self-attention within local windows during feature extraction for larger receptive fields and greater performance, compared to traditional CNN-based approaches. UFormer \cite{Uformer} introduces an innovative local-enhancement window Transformer block, utilizing a learnable multi-scale restoration modulator within the decoder to enhance the model's ability to detect both local and global patterns. ART \cite{ART} incorporates an attention retractable module to expand its receptive field, thereby enhancing SISR performance. CAT \cite{CAT} leverages rectangle-window self-attention for feature aggregation, achieving a broader receptive field. HAT \cite{HAT} integrates channel attention mechanism \cite{wang2020ecanet} with overlapping cross-attention module, leveraging more pixels to reconstruct better SISR results, thereby setting new benchmarks in the field.




\subsection{Auxiliary Supervision and Feature Fusion}

\textbf{Auxiliary Supervision.} Deep supervision is a commonly used auxiliary supervision method \cite{DeeplySupervised,szegedy2014going} that involves training by adding prediction layers at the intermediate levels of the model \cite{yolov9,CSPNET,ELAN}. This approach is particularly prevalent in architectures based on Transformers that incorporate multi-layer decoders. Another popular auxiliary supervision technique involves guiding the feature maps produced by the intermediate layers with relevant metadata to ensure they possess attributes beneficial to the target task \cite{guo2019augfpn,hayder2017boundaryaware,RRDB,RDB,huang2022monodtr}. Choosing the appropriate auxiliary supervision mechanism can accelerate the model's convergence speed, while also enhancing its robustness and performance.

\textbf{Feature Fusion.} Many studies have explored the integration of features across varying dimensions or multi-level features, such as FPN \cite{lin2017feature}, to obtain richer representations for different tasks \cite{RFA,Zamir2021Restormer}. In CNNs, attention mechanisms have been applied to both spatial and channel dimensions to improve feature representation; examples of which include RTCS \cite{RTCS} and SwinFusion \cite{SwinFusion}. In ViT \cite{VIT}, spatial self-attention is used to model the long-range dependencies between pixels. Additionally, some researchers have investigated the incorporation of channel attention within Transformers \cite{zhou2022understanding,chen2022mixformer} to effectively amalgamate spatial and channel information. This integration significantly enhances the modeling capabilities of Transformers.

==> sec/3_method.tex <==
\section{Methodology}
\label{sec:methodology}


\subsection{Network Architecture}

As shown in Figure \ref{DRCT.png}, DRCT comprises three distinct components: shallow feature extraction, deep feature extraction and image reconstruction module, respectively. 

\textbf{Shallow and deep feature extraction.} Given a low-resolution (LR) input $\mathbf{I}_{LR} \in \mathbb{R}^{H \times W \times C_{in}}$ ($H$, $W$ and $C_{in}$ are the image height, width and input channel number, respectively), we use a $3 \times 3$ convolutional layer $\text{Conv}$$(\cdot)$ \cite{xiao2021early} to extract shallow feature $\mathbf{F}_{\text{0}} \in \mathbb{R}^{H \times W \times C}$ as

\begin{equation}
\mathbf{F}_{\text{0}} = \text{Conv}(\mathbf{I}_{LQ}),
\end{equation}
 
Then, we extract deep feature which contains high-frequency spatial information \( \mathbf{F}_{DF} \in \mathbb{R}^{H \times W \times C} \) from \( \mathbf{F}_{\text{0}} \) and it can be defined as

\begin{equation}
\mathbf{F}_{DF} = H_{DF}(\mathbf{F}_0),
\end{equation}
where \( H_{DF}(\cdot) \) is the deep feature extraction module and it contains \( K \) Residual Deep feature extraction Group (RDG) and single convolutional layer $\text{Conv}(\cdot)$ for feature transition. More specifically, intermediate features \( \mathbf{F}_1, \mathbf{F}_2, \ldots, \mathbf{F}_K \) and the output deep feature \( \mathbf{F}_{DF} \) are extracted block by block as

\begin{equation}
 \mathbf{F}_i = \text{RDG}_{i}(\mathbf{F}_{i-1}), \quad i = 1, 2, \ldots, K,
\end{equation}

\begin{equation}
\mathbf{F}_{DF} = \text{Conv}(\mathbf{F}_K),
\end{equation}


\textbf{Image reconstruction.}
We reconstruct the SR image \( \mathbf{I}_{SR} \) $\in \mathbb{R}^{H \times W \times C_{in}}$ by aggregating shallow and deep features, it can be defined as:

\begin{equation}
\mathbf{I}_{SR} = H_{\text{rec}}(\mathbf{F}_0 + \mathbf{F}_{DF}),
\end{equation}
where \( H_{\text{rec}}(\cdot) \) is the function of the reconstruction for fusing high-frequency deep feature $\mathbf{F}_{DF}$ and low-frequency feature $\mathbf{F}_0$ together to obtain SR result.


\subsection{Deep Feature Extraction}

\textbf{Residual Deep feature extraction Group.} In developing of RDG, we take cues from RRDB-Net \cite{RRDB} and RDN \cite{RDB}, employing a residual-dense block (RDB) as the foundational unit for SISR. The reuse of feature maps emerges as the enhanced receptive field in the RDG's feed-forward mechanism. To expound further, RDG enhances the capability to integrate information across different scales, thus allowing for a more comprehensive feature extraction. Residual connections facilitate the flow of information, preventing the loss that often occurs in deep networks. This mechanism ensures that even as the depth of the network increases, essential details are preserved, effectively broadening the receptive field without compromising the integrity of the information.


\textbf{Swin-Dense-Residual-Connected Block.} In purpose of capturing the long-range dependency, we utilize the shifting window self-attention mechanism of Swin-Transformer Layer (STL) \cite{SwinTransformer,SwinIR} for obatining adaptive receptive fields, complementing RRDB-Net by focusing on multi-level spatial information. This synergy leverages STL to dynamically adjust the focus of the model based on the global content of the input, allowing for a more targeted and efficient extraction of features. By integrating STL with RRDB, the architecture benefits from both a vast receptive field and the capability to hone in on the most relevant information, thereby enhancing the model's performance in SISR tasks requiring detailed and context-aware processing. For the input feature maps $\mathbf{Z}$ within RDG, the SDRCB can be defined as:

\begin{equation}
\mathbf{Z}_j = H_{\text{trans}}(\text{STL}([\mathbf{Z}, ...,\mathbf{Z}_{j-1} ])), j = 1, 2, 3, 4, 5,
\end{equation}

%\begin{align*}
%    X_1 &= \text{PE}\left( \text{Conv}_{\sigma}\left(\text{PUE}\left(\text{STL}(X)\right)\right)\right) \\
%X_2 &= \text{PE}\left( \text{Conv}_{\sigma}\left(\text{PUE}\left(\text{STL}\left(\text{Cat.}(X, X_1), \right)\right)\right)\right) \\
%    X_3 &= \text{PE}\left( \text{Conv}_{\sigma}\left(\text{PUE}\left(\text{STL}\left(\text{Cat.}(X, X_1, X_2)\right)\right)\right)\right) \\
%    X_4 &= \text{PE}\left( 
%\text{Conv}_{\sigma}\left(\text{PUE}\left(\text{STL}\left(\text{Cat.}(X, X_1, X_2, X_3)\right)\right)\right)\right) \\
%    X_5 &= \text{PE}\left(           \text{Conv}_{1}\left(\text{PUE}\left(\text{STL}\left(\text{Cat.}(X, X_1, X_2, X_3, X_4)\right)\right)\right)\right) \\
%\end{align*}

\begin{equation}
\text{SDRCB}(\mathbf{Z}) =  \alpha \cdot \mathbf{Z}_5 + \mathbf{Z},
\end{equation}
where $[\cdot]$ denotes the concatenation of multi-level feature maps produced by the previously layers. \(H_{\text{trans}}(\cdot) \) refers to the convolutional layer with a LeakyReLU activate function for feature transition. The negative slope of LeakyReLU is set to $0.2$. $\text{Conv}_{1}$ is the $1 \times 1$ convolutional layer. $\alpha$ is residual scaling factor, which is set to $0.2$ for stabilizing the training process \cite{RRDB}.




\subsection{Same-task Progressive Training Strategy}

In recent years, Progressive Training Strategy (PTS) \cite{progressive,10208449} have gained increased attention and can be seen as a method of fine-tuning. Compared to conventional training methods, PTS tends to converge model parameters to more desirable local-minima. HAT \cite{HAT} introduces the concept of same-task pre-training, where training on a larger dataset like ImageNet \cite{imagenet} before fine-tuning on a specific dataset leads to improved SISR results. Lei \emph{et al.} \cite{L1L2} proposed initially training a SISR network with L1-loss and then using L2-loss to eliminate artifacts, achieving better results on the PSNR metric. This concept has been widely adopted \cite{ART}. Our proposed Same-task Progressive Training Strategy (SPTS), we first pre-trained DRCT on ImageNet to initialize model parameters and then fine-tuned on specific dataset with L1 loss as the optimization objective function, 

\begin{equation}
\ell_{L1}= \left\| I_{HR} - I_{SR} \right\|_1
\end{equation}

and finally use L2 loss to eliminate singular pixels and artifacts, therefore further archiving greater performance on PSNR metrics.

\begin{equation}
\ell_{L2}= \left\| I_{HR} - I_{SR} \right\|_2
\end{equation}


==> sec/4_5_futurework.tex <==
\section{Future Work}
\label{sec:future work}

In this section, we explore the potential areas for enhancement and future directions of development for DRCT, as described below.

\textbf{Generalizability.} Our proposed DRCT not only mitigates the negative impacts of information bottlenecks but also enhances the model's receptive field through feature fusion and auxiliary supervision within every single residual block by dense connection. We believe that adding dense connections within residual blocks holds potential for broader application across various low-level vision tasks due to their reliance on non-local priors for reconstruction. The core requirement for these tasks is capturing global information through an extensive receptive field.


\textbf{The upper-bound of model performance.} Given that the information bottlenecks mentioned earlier can be addressed through dense connections within residual blocks, DRCT is capable of achieving desirable performance with fewer parameters and a simpler model architecture. This suggests significant potential for further performance enhancements. For instance, meticulously designed window-attention mechanisms could be employed to broaden the model’s receptive field, or a greater focus could be placed on the interaction between features across different windows to enhance the model's feature extraction capabilities.

==> sec/4_experiment.tex <==
\section{Experiment Results}
\label{sec:experiment}

\begin{table*}[htbp]
\centering
\scalebox{0.92}{
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Method} & \textbf{Scale} & \textbf{Training} & \multicolumn{2}{c|}{\textbf{Set5} \cite{bevilacqua2012low}} & \multicolumn{2}{c|}{\textbf{Set14} \cite{10.1007/978-3-642-27413-8_47}} & \multicolumn{2}{c|}{\textbf{BSD100} \cite{937655}} & \multicolumn{2}{c|}{\textbf{Urban100} \cite{Huang-CVPR-2015}} & \multicolumn{2}{c|}{\textbf{Manga109} \cite{mtap_matsui_2017}} \\
\cline{4-13}
                &                &        \textbf{Dataset}                    & PSNR           & SSIM          & PSNR            & SSIM           & PSNR           & SSIM           & PSNR             & SSIM            & PSNR            & SSIM            \\
\hline

EDSR \cite{EDSR}  & $\times 2$     & DIV2K                      & 38.11          & 0.9602        & 33.92           & 0.9195         & 32.32          & 0.9013         & 32.93            & 0.9351          & 39.10           & 0.9773          \\
RCAN \cite{RCAN}  & $\times 2$     & DIV2K                      & 38.27          & 0.9614        & 34.12           & 0.9216         & 32.41          & 0.9027         & 33.34            & 0.9384          & 39.44           & 0.9786          \\

SAN \cite{dai2019second} & $\times 2$   & DIV2K & 38.31 & 0.9620 & 34.07 & 0.9213 & 32.42 & 0.9028 & 33.10 & 0.9370 & 39.32 & 0.9792 \\
IGNN \cite{zhou2020cross} & $\times 2$   & DIV2K & 38.24 & 0.9613 & 34.07 & 0.9217 & 32.41 & 0.9025 & 33.23 & 0.9383 & 39.35 & 0.9786 \\
HAN \cite{niu2020single} & $\times 2$   & DIV2K & 38.27 & 0.9614 & 34.16 & 0.9217 & 32.41 & 0.9027 & 33.35 & 0.9385 & 39.46 & 0.9785 \\
NLSN \cite{Mei_2021_CVPR} & $\times 2$   & DIV2K & 38.34 & 0.9618 & 34.08 & 0.9231 & 32.43 & 0.9027 & 33.42 & 0.9394 & 39.59 & 0.9789 \\
SwinIR \cite{SwinIR} & $\times 2$   & DF2K & 38.42 & 0.9623 & 34.46 & 0.9250 & 32.53 & 0.9041 & 33.81 & 0.9427 & 39.92 & 0.9797 \\
CAT-A \cite{CAT} & $\times 2$ & DF2K & 38.51 & 0.9626 & 34.78 & 0.9265 & 32.59 & 0.9047 & 34.26 & 0.9440 & 40.10 & 0.9805 \\
HAT \cite{HAT} & $\times 2$ & DF2K & 38.63 & 0.9630 & 34.86 & 0.9274 & 32.62 & 0.9053 & 34.45 & 0.9466 & 40.26 & 0.9809 \\  
DAT \cite{DAT} & $\times 2$ & DF2K & 38.58 &0.9629& 34.81& 0.9272& 32.61& 0.9051 &34.37 &0.9458& 40.33 &0.9807 \\
\textbf{DRCT (Ours)} & $\times 2$ & DF2K & \orange{\textbf{38.72}} & \blue{\textbf{0.9646}} & \orange{\textbf{34.96}} & \orange{\textbf{0.9287}} & \blue{\textbf{32.75}} & \blue{\textbf{0.9071}} & \orange{\textbf{34.54}} & \orange{\textbf{0.9474}} & \orange{\textbf{40.41}} & \orange{\textbf{0.9814}} \\\hdashline \hdashline 
IPT† \cite{IPT} & $\times 2$ & ImageNet & 38.37 & - & 34.43 & - & 32.48 & - & 33.76 & - & - &  - \\
EDT† \cite{EDT} & $\times 2$ & DF2K & 38.63 & 0.9632 & 34.80 & 0.9273 & 32.62 & 0.9052 & 34.27 & 0.9456 & 40.37 & 0.9811 \\
HAT-L$\dagger$ \cite{HAT} & $\times 2$ & DF2K & \blue{38.91} & \blue{0.9646} & \blue{35.29} & \blue{0.9293} & \orange{32.74} & \orange{0.9066} & \blue{35.09} & \blue{0.950}5 & \blue{41.01} & \blue{0.9831} \\
\textbf{DRCT-L$\ddagger$ (Ours)} & $\times 2$ & DF2K & \red{\textbf{39.14}} & \red{\textbf{0.9658}} & \red{\textbf{35.36}} & \red{\textbf{0.9302}} & \red{\textbf{32.90}} & \red{\textbf{0.9078}} & \red{\textbf{35.17}} & \red{\textbf{0.9516}} & \red{\textbf{41.14}} & \red{\textbf{0.9842}} \\
%... continue with other rows
\hline

EDSR \cite{EDSR}  & $\times 3$ & DIV2K & 34.65 & 0.9280 & 30.52 & 0.8462 & 29.25 & 0.8093 & 28.80 & 0.8653 & 34.17 & 0.9476 \\
RCAN \cite{RCAN}& $\times 3$ & DIV2K & 34.74 & 0.9299 & 30.65 & 0.8482 & 29.32 & 0.8111 & 29.09 & 0.8702 & 34.44 & 0.9499 \\
SAN \cite{dai2019second}& $\times 3$ & DIV2K & 34.75 & 0.9300 & 30.59 & 0.8476 & 29.33 & 0.8112 & 28.93 & 0.8671 & 34.30 & 0.9494 \\
IGNN \cite{zhou2020cross}& $\times 3$ & DIV2K & 34.72 & 0.9298 & 30.66 & 0.8484 & 29.31 & 0.8105 & 29.03 & 0.8696 & 34.39 & 0.9496 \\
HAN \cite{niu2020single}& $\times 3$ & DIV2K & 34.75 & 0.9299 & 30.67 & 0.8483 & 29.32 & 0.8110 & 29.10 & 0.8705 & 34.48 & 0.9500 \\
NLSN \cite{Mei_2021_CVPR}& $\times 3$ & DIV2K & 34.85 & 0.9306 & 30.70 & 0.8485 & 29.34 & 0.8117 & 29.25 & 0.8726 & 34.57 & 0.9508 \\
SwinIR \cite{SwinIR}& $\times 3$ & DF2K & 34.97 & 0.9318 & 30.93 & 0.8534 & 29.46 & 0.8145 & 29.75 & 0.8826 & 35.12 & 0.9537 \\ 
CAT-A \cite{CAT} &  $\times 3$ & DF2K & 35.06 & 0.9326 & 31.04 & 0.8538 & 29.52 & 0.8160 & 30.12 & 0.8862  &35.38  &0.9546 \\

HAT \cite{HAT} & $\times 3$ & DF2K & 35.07 & 0.9329 & 31.08 & 0.8555 & 29.54 & 0.8167 & 30.23 & 0.8896 & 35.53 & 0.9552 \\ 

DAT \cite{DAT} & $\times 3$ & DF2K&35.16 &0.9331 &31.11 &0.8550 & 29.55 & 0.8169 & 30.18& 0.8886 &35.59 &0.9554 \\

\textbf{DRCT (Ours)} & $\times 3$ & DF2K & \orange{\textbf{35.18}} & \orange{\textbf{0.9338}} & \orange{\textbf{31.24}} & \orange{\textbf{0.8569}} & \blue{\textbf{29.68}} & \orange{\textbf{0.8182}} & \orange{\textbf{30.34}} & \orange{\textbf{0.8910}} & \orange{\textbf{35.76}} & \orange{\textbf{0.9575}} \\\hdashline \hdashline 
IPT† \cite{IPT}  & $\times 3$ & ImageNet & 34.87 & - & 30.85 & - & 29.38 & - & 29.49 & - & - & - \\
EDT† \cite{EDT}& $\times 3$ & DF2K & 35.13 & 0.9328 & 31.09 & 0.8553 & 29.53 & 0.8165 & 30.07 & 0.8863 & 35.47 & 0.9550 \\
HAT-L$\dagger$ \cite{HAT} & $\times 3$ & DF2K & \blue{35.28} & \blue{0.9345} & \blue{31.47} & \blue{0.8584} & \orange{29.63} & \blue{0.8191} & \blue{30.92} & \blue{0.8981} & \blue{36.02} & \blue{0.9576} \\
\textbf{DRCT-L$\ddagger$ (Ours)} & $\times 3$ & DF2K & \red{\textbf{35.32}} & \red{\textbf{0.9348}} & \red{\textbf{31.54}} & \red{\textbf{0.8591}} & \red{\textbf{29.68}} & \red{\textbf{0.8211}} & \red{\textbf{31.14}} & \red{\textbf{0.9004}} & \red{\textbf{36.16}} & \red{\textbf{0.9585}} \\

\hline



EDSR \cite{EDSR} & $\times 4$ & DIV2K & 32.46 & 0.8968 & 28.80 & 0.7876 & 27.71 & 0.7420 & 26.64 & 0.8033 & 31.02&0.9148 \\
RCAN \cite{RCAN}& $\times 4$ & DIV2K & 32.63 & 0.9002 & 28.87 & 0.7889 & 27.77 & 0.7436 & 26.82 & 0.8087 & 31.22&0.9173 \\
SAN \cite{dai2019second}& $\times 4$ & DIV2K & 32.64 & 0.9003 & 28.92 & 0.7888 & 27.78 & 0.7436 & 26.79 & 0.8068 & 31.18&0.9169 \\
IGNN \cite{zhou2020cross}& $\times 4$ & DIV2K & 32.57 & 0.8998 & 28.85 & 0.7891 & 27.77 & 0.7434 & 26.84 & 0.8090 & 31.28&0.9182 \\
HAN \cite{niu2020single}& $\times 4$ & DIV2K & 32.64 & 0.9002 & 28.90 & 0.7890 & 27.80 & 0.7442 & 26.85 & 0.8094 & 31.42&0.9177 \\
NLSN \cite{Mei_2021_CVPR}& $\times 4$ & DIV2K & 32.59 & 0.9000 & 28.87 & 0.7891 & 27.78 & 0.7444 & 26.96 & 0.8109 & 31.27&0.9184 \\
SwinIR \cite{SwinIR}& $\times 4$ & DF2K & 32.92 & 0.9044 & 29.09 & 0.7950 & 27.92 & 0.7489 & 27.45 & 0.8254 & 32.03&0.9260 \\
CAT-A \cite{CAT} &  $\times 4$ & DF2K & 33.08 & 0.9052 & 29.18 & 0.7960 & 27.99 & 0.7510 & 27.89 & 0.8339 & 32.39 & 0.9285 \\

HAT  \cite{HAT}& $\times 4$ & DF2K & 33.04 & 0.9056 & 29.23 & 0.7973 & 28.00 & 0.7517 & 27.97 & 0.8368 & 32.48& 0.9292 \\

DAT \cite{DAT} & $\times 4$ & DF2K & 33.08& 0.9055& 29.23& 0.7973& 28.00 &0.7515& 27.87& 0.8343 &32.51 &0.9291\\
\textbf{DRCT (Ours)} & $\times 4$ & DF2K & \orange{\textbf{33.11}} & \orange{\textbf{0.9064}} & \orange{\textbf{29.35}} & \orange{\textbf{0.7984}} & \blue{\textbf{28.18}} & \orange{\textbf{0.7532}} & \orange{\textbf{28.06}} & \orange{\textbf{0.8378}} & \orange{\textbf{32.59}} & \orange{\textbf{0.9304}} \\\hdashline \hdashline 

IPT† \cite{IPT}  & $\times 4$ & ImageNet & 32.64 & - & 29.01 & - & 27.82 & - & 27.26 & - & -  & - \\
EDT† \cite{EDT}& $\times 4$ & DF2K & 32.82 & 0.9031 & 29.09 & 0.7939 & 27.91 & 0.7483 & 27.46 & 0.8246 & 32.05&0.9254 \\
HAT-L$\dagger$ \cite{HAT} & $\times 4$ & DF2K & \blue{33.30} & \blue{0.9083} & \blue{29.47} & \blue{0.8015} & \orange{28.09} & \blue{0.7551} & \blue{28.60} & \blue{0.8498} & \blue{33.09} & \blue{0.9335} \\
\textbf{DRCT-L$\ddagger$ (Ours)} & $\times 4$ & DF2K & \red{\textbf{33.37}} & \red{\textbf{0.9090}} & \red{\textbf{29.54}} & \red{\textbf{0.8025}} & \red{\textbf{28.16}} & \red{\textbf{0.7577}} & \red{\textbf{28.70}} & \red{\textbf{0.8508}} & \red{\textbf{33.14}} & \red{\textbf{0.9347}} \\
\hline
\end{tabular}}
\caption{Quantitative comparison with the several peer-methods on benchmark datasets. "$\dagger$” indicates that methods adopt pre-training strategy \cite{HAT} on ImageNet. "$\ddagger$” represents that methods use same-task progressive-training strategy. The top three results are marked in \red{\textbf{red}}, \blue{\textbf{blue}}, and \orange{\textbf{orange}} , respectively.}
\label{quantitative}
\end{table*}


\begin{figure*}
\includegraphics[width=1\textwidth]{fig/RESULT3.png}
\caption{Visual comparison on × 4 SISR. The patches for comparison are marked with red boxes in the original images. The higher the PSNR/SSIM metrics, the better the performance..} \label{RESULT1.png}
\end{figure*}


\subsection{Dataset}

Our DRCT model is trained on DF2K, a substantial aggregated dataset that includes DIV2K \cite{Agustsson_2017_CVPR_Workshops} and Flickr2K \cite{Timofte_2017_CVPR_Workshops}. DIV2K provides 800 images for training, while Flickr2K contributes a larger set of 2650 images. For the training input, we generate low-resolution versions of these images by applying a bicubic downsampling method with scaling factors of $2$, $3$, and $4$, respectively. To assess the effectiveness of our model, we conduct performance evaluations using well-known Image Super-Resolution benchmark datasets such as Set5 \cite{bevilacqua2012low}, Set14 \cite{10.1007/978-3-642-27413-8_47}, BSD100 \cite{937655}, Urban100 \cite{Huang-CVPR-2015}, and Manga109 \cite{mtap_matsui_2017}, which are standard in SISR tasks.

\subsection{Implementation Details}
               
The training process can be structured into three distinct phases, as ullustrated as Section 4-3. (1) pre-trained on ImageNet \cite{imagenet}, (2) optimize the model on the given dataset, (3) L2-loss for PSNR enhancement. Throughout the training process, we use the Adam optimizer with $\beta_{1}$ = $0.9$, and $\beta_{2}$ = $0.999$ and train for $800k$ iterations in first and second stage. The learning rate is set to $2e-4$, the multi-step learning scheduler is also used. The learning rate is halved at the $300k$, $500k$, $650k$, $700k$, $750k$ iterations respectively. Weight decay is not applied and the batch-size is set to $32$. In the architecture of DRCT, the configuration of depth and width is maintained identically to that of HAT \cite{HAT}. To elaborate, both the number of RDG and SDRCB units are established at 6, and the channel number of intermediate feature maps is designated as 180. The attention head number and window size are set to 6 and 16 for window-based multi head self-attention (W-MSA). In terms of data preparation, HR patches with dimensions of $256$ $\times$ $256$ pixels were extracted from the HR images. To improve the generalizability, we apply random horizontal flips and rotation augmentation.




\subsection{Quantitative Results} For the evaluation, we use full RGB channels and ignore the \( (2 \times \text{scale}) \) pixels from the border. PSNR and SSIM metrics are used to evaluation criteria. Table \ref{quantitative} presents the quantitative comparison of our approach and the state-of-the-art methods, including EDSR \cite{EDSR}, RCAN \cite{RCAN}, SAN \cite{dai2019second}, IGN \cite{zhou2020cross}, HAN \cite{niu2020single}, NLSN \cite{Mei_2021_CVPR}, SwinIR \cite{SwinIR}, CAT-A \cite{CAT}, DAT \cite{DAT}, as well as approaches using ImageNet pre-training, such as IPT \cite{IPT}, EDT \cite{EDT} and HAT \cite{HAT}. We can see that our method outperforms the other methods significantly on all benchmark datasets. In addition, the DRCT-L can bring further improvement and greatly expands the performance upper-bound of this task. Even with fewer model parameters and computational requirements, DRCT is also significantly greater than the state-of-the-art methods. 

\subsection{Visual Comparison} The visual comparisons displayed in Figure \ref{RESULT1.png}. For the selected images from the Urban100 \cite{Huang-CVPR-2015}, DRCT is effective in restoring structures, whereas other methods suffer from notably blurry effects. The visual results demonstrate the superiority of our approach.

Along with providing visualizations for the LAM \cite{LAM}, we compute the DI and GI. In scenarios where DRCT operates with fewer parameters (a topic for the next subsection), it achieves a higher DI. This outcome suggests that, after enhancing the receptive field through SDRCB, the model can leverage a greater amount of non-local information for SISR without the need for intricately designed W-MSA. Additionally, the GI of the proposed DRCT, being the lowest among the three, underscores its training process stability and its effectiveness in minimizing information loss.


There remains significant room for improvement in the way information loss is measured for SISR models. We conducted a detailed analysis of the G-index using 'image\_092' from Urban100, as shown in Figure \ref{LAM2.png}. DRCT managed to achieve a lower score on the GI, indicating that the changes in the network's feature maps are relatively stable. In contrast, The GI for HAT was significantly higher than the other two, which suggests that a lower GI value can effectively denote lesser information loss, whereas a higher GI might imply more drastic changes in feature maps. However, this doesn't necessarily correlate directly with the effectiveness of measuring information loss.

\begin{figure}
\includegraphics[width=0.5\textwidth]{fig/featuremap7.png}
\caption{The LAM \cite{LAM} visualization. DRCT improves performance by enhancing the receptive field to mitigate the issue of spatial information loss in deeper layers of the network. 
%(zoom in to better see the color-bar of feature maps.)
} \label{LAM2.png}
\end{figure}

\begin{figure}
\includegraphics[width=0.5\textwidth]{fig/complexity.png}
\caption{The model complexity comparison between SwinIR, HAT, and proposed DRCT evaluated on Urban100 \cite{Huang-CVPR-2015} dataset.} \label{complexity.png}
\end{figure}



\subsection{Model Complexity}

To demonstrate the potential of our proposed method, we conducted further analysis on model complexity, with the results illustrated in Figure \ref{complexity.png}. From the figure, we can observe that the performance curves of the HAT and SwinIR models are approaching horizontal lines, suggesting that their model performance is nearing a bottleneck. Enhancing performance may require more sophisticated design or a greater number of parameters, potentially leading to prohibitive costs and practical implementation challenges. In contrast, our DRCT-L model outperforms HAT-L while saving 33\% of model parameters. This indicates that stabilizing the training and inference processes within residual blocks through a dense-group is a viable strategy to prevent SISR models from encountering information bottlenecks.

\subsection{NTIRE Image Super-Resolution (x4) Challenge}

\begin{table}[ht]
\centering
\begin{tabular}{lcc}
\toprule
      & Validation phase & Testing phase \\
\midrule
PSNR  & 31.8201           & 31.7784         \\
SSIM  & 0.8494            & 0.8655          \\
\bottomrule
\end{tabular}
\caption{NTIRE 2024 Challenge Results with x4 SR in terms of PSNR and SSIM on validation phase and testing phase.}
\label{ntire2024}
\end{table}


The dataset for the NTIRE 2024 Image Super-Resolution (x4) Challenge \cite{chen2024ntire_sr} comprises three collections: DIV2K \cite{Agustsson_2017_CVPR_Workshops}, Flickr2K \cite{Timofte_2017_CVPR_Workshops}, and LSDIR \cite{Li_2023_CVPR}. Specifically, the DIV2K dataset provides 800 pairs of HR and LR images for training. The LR images are obtained from the HR images after bicubic downsampling with specific scaling factor. For validation, it offers 100 LR images for the purpose of creating SR images, with the HR versions to be made available at the challenge's final stage. Additionally, the test dataset includes 100 varied LR images. The self-ensemble strategy is used for testing-time augmentation (TTA) \cite{timofte2015seven}. Our TTA methods include random rotation, and horizontal and vertical flipping. We also conducted a model ensemble strategy for fusing different reconstructed results by HAT \cite{HAT} and the proposed DRCT to eliminate the annoying artifacts and improve final SR quality. Our SISR model was entered into both the validation and testing phases of this challenge, with the detailed in Table \ref{ntire2024}.





==> sec/5_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}


In this paper, we introduce the phenomenon of information bottlenecks observed in SISR models, where spatial information is lost as network depth increases during the forward-propagation. This may lead to information loss when back-propagation and severe oscillations in the distribution of feature intensities, limiting the upper-bound of model performance for the SISR task requiring detailed spatial information and context-aware processing.

To address these issues, we present a novel Swin-transformer-based model named the Dense-residual-connected Transformer (DRCT). The design philosophy behind DRCT centers on stabilizing the forward-propagation process and enhancing the receptive fields by incorporating dense-connections within residual blocks, combining the shift-window attention mechanism to adaptively capture global information. This approach reduces the loss of spatial information, addressing the information bottleneck that SISR models may encounter in deeper network layers.

As a result, the model can better focus on global spatial information and surpass existing state-of-the-art methods without the need for designing sophisticated window attention mechanisms or increasing model parameters. The experiment results have demonstrated that the efficacy of proposed DRCT, indicating its effectiveness and the potential of the future work.






